Luminosities and masses of single Galactic Post-Asymptotic Giant Branch (Post-AGB) stars with distances from $Gaia$ EDR3: The revelation of an $s$-process diversity

Post-AGB stars are exquisite probes of AGB nucleosynthesis. However, the previous lack of accurate distances jeopardised comparison with theoretical AGB models. The $Gaia$ Early Data Release 3 ($Gaia$ EDR3) has now allowed for a breakthrough in this research landscape. In this study, we focus on a sample of single Galactic post-AGBs for which chemical abundance studies were completed. We combined photometry with geometric distances to carry out a spectral energy distribution (SED) analysis and derive accurate luminosities. We subsequently determined their positions on the HR-diagram and compared this with theoretical post-AGB evolutionary tracks. While most objects are in the post-AGB phase of evolution, we found a subset of low-luminosity objects that are likely to be in the post-horizontal branch phase of evolution, similar to AGB-manqu\'e objects found in globular clusters. Additionally, we also investigated the observed bi-modality in the $s$-process enrichment of Galactic post-AGB single stars of similar Teff, and metallicities. This bi-modality was expected to be a direct consequence of luminosity with the $s$-process rich objects having evolved further on the AGB. However, we find that the two populations: the $s$-process enriched and non-enriched, have similar luminosities (and hence initial masses), revealing an intriguing chemical diversity. For a given initial mass and metallicity, AGB nucleosynthesis appears inhomogeneous and sensitive to other factors which could be mass-loss, along with convective and non-convective mixing mechanisms. Modelling individual objects in detail will be needed to investigate which parameters and processes dominate the photospheric chemical enrichment in these stars.

==> Table1_v1.tex <==
\begin{longrotatetable}
\begin{deluxetable*}{rrrrrrrrrrrrrr}
\tabletypesize{\footnotesize}
\tablecolumns{14}
\tablewidth{0pt}
%\small
\tabletypesize{\scriptsize}
\setlength{\tabcolsep}{3pt}
\tablecaption{Fundamental properties of the $s$-process rich and non-enriched single Galactic post-AGB stars. See Section~\ref{sec:lum+mass} for more details. \label{table1}}
\tablehead{
%\colhead{Index} & \colhead{Object Name} & \colhead{Parallax(mas)} & \colhead{Error(mas)} & \colhead{$z_{\rm 1/parallax}$(pc)} & \colhead{$z_{\rm BJ}$(pc)} & \colhead{$z_{\rm BJL}$(pc)} & \colhead{$z_{\rm BJU}$(pc)} & \colhead{\Teff(K)} & \colhead{E$(B-V)$} & \colhead{L/\Lsun} & \colhead{L$_{\rm Lower}$/\Lsun} & \colhead{L$_{\rm Upper}$/\Lsun} \\
\colhead{Index} & \colhead{Object Name} & \colhead{Parallax} & \colhead{Error} & \colhead{$z_{\rm 1/parallax}$} & \colhead{$z_{\rm BJ}$} & \colhead{$z_{\rm BJL}$} & \colhead{$z_{\rm BJU}$} & \colhead{\Teff} & \colhead{\logg} &\colhead{E($B-V$)} & \colhead{L/\Lsun} & \colhead{L$_{\rm Lower}$/\Lsun} & \colhead{L$_{\rm Upper}$/\Lsun} \\
\colhead{} & \colhead{} & \colhead{(mas)} & \colhead{(mas)} & \colhead{(pc)} & \colhead{(pc)} & \colhead{(pc)} & \colhead{(pc)} & \colhead{(K)} & \colhead{(dex)} & \colhead{} & \colhead{} & \colhead{} & \colhead{} \\
%
%\colhead{} & \colhead{} & \colhead{} & \colhead{} &  \colhead{} & \colhead{(J2000)} & \colhead{(J2000)} & \colhead{(mas)} & \colhead{(mas)} & \colhead{(pc)} & \colhead{(pc)}& \colhead{(pc)} & \colhead{(pc)} & \colhead{(K)} & \colhead{} & \colhead{(\Lsun)} & \colhead{(\Lsun)} & \colhead{(\Lsun)}
} 
\startdata
\multicolumn{14}{c}{Post-AGB stars with$s$-process enrichment}\\
\hline
1	&	IRASZ02229+6208	&	0.38	&	0.06	&	2627.53	&	2352.18	&	2063.48	&	2687.03	&	5952 $\pm$ 250	&	0.00	&	1.9$^{+0.08}_{-0.42}$	&	12959	&	9973	&	16911	\\
2	&	IRAS04296+3429	&	-0.38	&	0.17	&	-2635.11	&	5048.41	&	3899.38	&	7150.92	&	7272 $\pm$ 250	&	0.73	&	2.03	&	10009	&	5971	&	20082	\\
3	&	IRAS05113+1347	&	-0.01	&	0.15	&	-108371.7	&	4629.82	&	3312.65	&	8416.2	&	5025 $\pm$ 250	&	0.01	&	0.75	&	2037	&	1043	&	6731	\\
4	&	IRAS05341+0852	&	0.51	&	0.19	&	1960.07	&	2057.38	&	1603.89	&	2778.95	&	6274 $\pm$ 250	&	0.84	&	1.18	&	324	&	197	&	592	\\
5	&	IRAS06530-0213	&	0.24	&	0.07	&	4145.93	&	3777.67	&	2886.46	&	4990.04	&	7809 $\pm$ 250	&	1.70	&	1.85	&	4687	&	2736	&	8178	\\
6	&	IRAS07134+1005	&	0.45	&	0.02	&	2203.76	&	2099.09	&	1991.41	&	2209.25	&	7485 $\pm$ 250	&	0.50	&	0.43	&	5505	&	4955	&	6098	\\
7	&	IRAS07430+1115	&	3.06	&	0.5	&	327.04	&	360.93	&	299.59	&	442.65	&	5519 $\pm$ 250	&	1.43	&	1.04	&	20	&	14	&	30	\\
8	&	IRAS08143-4406	&	0.24	&	0.02	&	4198.54	&	4154.69	&	3877.12	&	4568.46	&	7013 $\pm$ 250	&	1.31	&	1.53	&	4509	&	3927	&	5452	\\
9	&	IRAS08281-4850	&	-0.14	&	0.07	&	-7300.68	&	11452.58	&	8728.27	&	15113.73	&	7462 $\pm$ 250	&	1.04	&	1.23	&	9584	&	5567	&	16692	\\
10	&	IRAS12360-5740	&	0.09	&	0.01	&	10970.73	&	9082.07	&	8261.41	&	10230.48	&	7273 $\pm$ 250	&	1.59	&	1.01	&	6258	&	5178	&	7940	\\
11	&	IRAS13245-5036	&	0.01	&	0.02	&	85919.8	&	14207.28	&	11305.73	&	17383.96	&	9037 $\pm$ 250	&	3.20	&	0.64	&	11221	&	7106	&	16800	\\
12	&	IRAS14325-6428	&	0.19	&	0.04	&	5220.46	&	4883.39	&	4261.63	&	5811.07	&	7256 $\pm$ 250	&	1.00	&	1.07	&	4935	&	3758	&	6988	\\
13	&	IRAS14429-4539	&	-0.11	&	0.51	&	-9372.15	&	3847.71	&	2160.1	&	6548.2	&	9579 $\pm$ 250	&	2.48	&	2.63	&	5049	&	1591	&	14624	\\
14	&	IRAS19500-1709	&	0.4	&	0.03	&	2504.9	&	2310.24	&	2164.96	&	2481.49	&	8239 $\pm$ 250	&	1.08	&	0.56	&	7053	&	6194	&	8138	\\
15	&	IRAS20000+3239	&	0.2	&	0.05	&	4880.07	&	4581.29	&	3695.53	&	6075.01	&	5478 $\pm$ 250	&	0.13	&	1.76	&	14342	&	9332	&	25218	\\
16	&	IRAS22223+4327	&	0.33	&	0.03	&	3007.27	&	2678.03	&	2546.9	&	2878.56	&	6008 $\pm$ 250	&	1.05	&	0.43	&	2163	&	1956	&	2499	\\
17	&	IRAS22272+5435	&	0.69	&	0.03	&	1457.75	&	1409.84	&	1355.87	&	1464.67	&	5325 $\pm$ 250	&	0.77	&	0.88	&	5659	&	5234	&	6108	\\
18	&	IRAS23304+6147	&	0.24	&	0.03	&	4226.42	&	3979.67	&	3620.05	&	4390.37	&	6276 $\pm$ 250	&	0.78	&	1.83	&	7712	&	6381	&	9386	\\		
\hline
\multicolumn{14}{c}{Post-AGB stars without $s$-process enrichment}\\ 
\hline
19	&	IRAS01259+6823	&	0.62	&	0.14	&	1624.61	&	1781.38	&	1434.96	&	2456.33	&	5510 $\pm$ 250	&	2.5	&	1.02	&	340	&	220	&	646	\\
20	&	IRAS08187-1905	&	0.29	&	0.03	&	3473.16	&	3258.96	&	2917.24	&	3649.91	&	5772 $\pm$ 250	&	0.98	&	0.07	&	2619	&	2099	&	3286	\\
21	&	SAO 239853	&	-0.01	&	0.07	&	-117255.41	&	8691.08	&	6485.52	&	12490.93	&	7452 $\pm$ 250	&	1.49	&	0.3	&	23490	&	13080	&	48520	\\
22	&	HD107369	&	0.37	&	0.02	&	2725.26	&	2568.38	&	2429.15	&	2705.92	&	7533 $\pm$ 250	&	2.45	&	0.07	&	910	&	814	&	1010	\\
23	&	HD 112374	&	0.57	&	0.02	&	1763.78	&	1684.48	&	1619.4	&	1768.68	&	6393 $\pm$ 250	&	0.80	&	0.3	&	10777	&	9961	&	11882	\\
24	&	HD133656	&	0.56	&	0.03	&	1776.54	&	1707.63	&	1646.84	&	1781.63	&	8238 $\pm$ 250	&	1.38	&	0.29	&	5227	&	4861	&	5690	\\
25	&	HR 6144	&	0.28	&	0.03	&	3561.19	&	3101.16	&	2894.87	&	3387.69	&	6728 $\pm$ 250	&	0.93	&	0.11	&	25491	&	22212	&	30419	\\
26	&	HD161796	&	0.5	&	0.02	&	1991.19	&	1920.96	&	1829.56	&	2015.66	&	6139 $\pm$ 250	&	0.99	&	0.13	&	5742	&	5209	&	6322	\\
27	&	IRAS18025-3906	&	0.54	&	0.19	&	1865.62	&	3046.67	&	1973.6	&	7194.98	&	6154 $\pm$ 250	&	1.18	&	0.96	&	2324	&	975	&	12963	\\
28	&	HD335675	&	0.03	&	0.18	&	30507.45	&	4888.53	&	3319.14	&	6540.55	&	6082 $\pm$ 250	&	1.58	&	0.85	&	15843	&	7303	&	28359	\\
29	&	IRAS19386+0155	&	0.32	&	0.16	&	3088.79	&	3631.35	&	2441.76	&	5588.81	&	6303 $\pm$ 250	&	1.00	&	1.23	&	9611	&	4345	&	22765	\\
30	&	IRAS19475+3119	&	0.32	&	0.02	&	3165.15	&	2971.43	&	2785.82	&	3135.57	&	8216 $\pm$ 250	&	1.01	&	0.61	&	6775	&	5955	&	7545	\\
31	&	HR7671	&	1.34	&	0.03	&	748.77	&	727.4	&	714.04	&	742.99	&	6985 $\pm$ 250	&	0.83	&	0.4	&	3579	&	3449	&	3734	\\
\enddata
%\tablenotetext{1}{Footnote}
\end{deluxetable*}
\end{longrotatetable}


==> Table3_v1.tex <==
\begin{longrotatetable}
\begin{deluxetable*}{rrrrrrrrrrrrrr}
\tabletypesize{\footnotesize}
\tablecolumns{14}
\tablewidth{0pt}
\small
\tabletypesize{\scriptsize}
\setlength{\tabcolsep}{3pt}
\tablecaption{Chemical abundances of the $s$-process enriched and non $s$-process enriched single Galactic post-AGB stars. \label{table3}}
%\vspace*{-\baselineskip}
%\small
%\tablecaption{Chemical abundances of the $s$-process enriched and non $s$-process enriched single Galactic post-AGB stars.\label{table2}}
%\tablewidth{700pt}
%\tabletypesize{\scriptsize}
%\setlength{\tabcolsep}{3.5pt}
\tablehead{
\colhead{Index} & \colhead{Object Name} & \colhead{\feh} & \colhead{\co} & \colhead{\ofe} & \colhead{\cfe} & 
\colhead{\nfe} & \colhead{\sfe} & \colhead{\Sfe} & \colhead{\zrfe} & \colhead{\lsfe} & \colhead{\hsfe} & \colhead{\hsls} & \colhead{Ref.}
} 
\startdata
\multicolumn{14}{c}{Post-AGB stars with $s$-process enrichment}\\ 
\hline
1	&	IRASZ02229+6208	&	-0.45 $\pm$ 0.14	&	\nodata	&	\nodata	&	0.78 $\pm$ 0.15	&	1.19 $\pm$ 0.30	&	1.4 $\pm$ 0.15	&	0.35 $\pm$ 0.14	&	2.22 $\pm$ 0.13	&	2.03 $\pm$ 0.12	&	1.12 $\pm$ 0.03	&	-0.91 $\pm$ 0.12	&	1	\\
2	&	IRAS04296+3429	&	-0.62 $\pm$ 0.11	&	\nodata	&	\nodata	&	0.8 $\pm$ 0.2	&	0.39 $\pm$ 0.01	&	1.5 $\pm$ 0.23	&	0.43	&	1.34 $\pm$ 0.23	&	1.7 $\pm$ 0.23	&	1.5 $\pm$ 0.17	&	-0.2 $\pm$ 0.23	&	2	\\
3	&	IRAS05113+1347	&	–0.49 $\pm$ 0.15	&	2.42 $\pm$ 0.40	&	0.01 $\pm$ 0.27	&	0.65 $\pm$ 0.16	&	\nodata	&	1.54 $\pm$ 0.07	&	0.06 $\pm$ 0.25	&	1.36 $\pm$ 0.15	&	1.33 $\pm$ 0.13	&	1.65 $\pm$ 0.07	&	0.32 $\pm$ 0.15	&	3	\\
4	&	IRAS05341+0852	&	–0.54 $\pm$ 0.11	&	1.06 $\pm$ 0.30	&	0.75 $\pm$ 0.11	&	1.03 $\pm$ 0.10	&	\nodata	&	2.12 $\pm$ 0.05	&	0.25 $\pm$ 0.15	&	1.76 $\pm$ 0.10	&	1.87 $\pm$ 0.08	&	2.24 $\pm$ 0.06	&	0.37 $\pm$ 0.10	&	3	\\
5	&	IRAS06530-0213	&	–0.32 $\pm$ 0.11	&	1.66 $\pm$ 0.39	&	0.35 $\pm$ 0.11	&	0.83 $\pm$ 0.13	&	\nodata	&	1.94 $\pm$ 0.06	&	0.21 $\pm$ 0.18	&	1.60 $\pm$ 0.10	&	1.75 $\pm$ 0.09	&	2.04 $\pm$ 0.08	&	0.29 $\pm$ 0.13	&	3	\\
6	&	IRAS07134+1005	&	–0.91 $\pm$ 0.20	&	1.24 $\pm$ 0.29	&	0.81 $\pm$ 0.19	&	1.16 $\pm$ 0.22	&	0.57 $\pm$ 0.19	&	1.63 $\pm$ 0.14	&	0.38 $\pm$ 0.24	&	1.61 $\pm$ 0.09	&	1.64 $\pm$ 0.13	&	1.63 $\pm$ 0.20	&	–0.01 $\pm$ 0.24	&	3	\\
7	&	IRAS07430+1115	&	–0.31 $\pm$ 0.15	&	1.71 $\pm$ 0.30	&	0.30  $\pm$ 0.22	&	0.79 $\pm$ 0.13	&	\nodata	&	1.47 $\pm$ 0.06	&	-0.08 $\pm$ 0.13	&	1.22 $\pm$ 0.15	&	1.30 $\pm$ 0.14	&	1.55 $\pm$ 0.06	&	0.25 $\pm$ 0.15	&	3	\\
8	&	IRAS08143-4406	&	–0.43 $\pm$ 0.11	&	1.66 $\pm$ 0.39	&	0.19 $\pm$ 0.13	&	0.71 $\pm$ 0.10	&	0.01 $\pm$ 0.22	&	1.65 $\pm$ 0.05	&	0.41 $\pm$ 0.14	&	1.63 $\pm$ 0.11	&	1.77 $\pm$ 0.08	&	1.58 $\pm$ 0.06	&	–0.19 $\pm$ 0.11	&	3	\\
9	&	IRAS08281-4850	&	–0.26 $\pm$ 0.11	&	2.34 $\pm$ 0.42	&	0.12 $\pm$ 0.11	&	0.75 $\pm$ 0.21	&	\nodata	&	1.58 $\pm$ 0.09	&	0.38 $\pm$ 0.24	&	1.42 $\pm$ 0.11	&	1.57 $\pm$ 0.11	&	1.58 $\pm$ 0.12	&	0.01 $\pm$ 0.17	&	3	\\
10	&	IRAS12360-5740	&	−0.40$\pm$0.15	&	0.45 $\pm$ 0.20	&	0.31 $\pm$ 0.05	&	0.27 $\pm$ 0.18	&	0.22 $\pm$ 0.32	&	1.88 $\pm$ 0.20	&	0.23 $\pm$ 0.16	&	1.70 $\pm$ 0.17	&	1.73 $\pm$ 0.20	&	2.02 $\pm$ 0.20	&	0.29 $\pm$ 0.20	&	4	\\
11	&	IRAS13245-5036	&	–0.30 $\pm$ 0.10	&	1.11 $\pm$ 0.30	&	0.26 $\pm$ 0.13	&	0.57 $\pm$ 0.21	&	\nodata	&	1.88 $\pm$ 0.09	&	\nodata	&	1.72 $\pm$ 0.15	&	1.56 $\pm$ 0.14	&	2.03 $\pm$ 0.11	&	0.47 $\pm$ 0.18	&	3	\\
12	&	IRAS14325-6428	&	–0.56 $\pm$ 0.10	&	2.27 $\pm$ 0.40	&	0.57 $\pm$ 0.09	&	1.18 $\pm$ 0.23	&	0.18 $\pm$ 0.20	&	1.30 $\pm$ 0.14	&	0.64 $\pm$ 0.32	&	1.16 $\pm$ 0.16	&	1.25 $\pm$ 0.15	&	1.33 $\pm$ 0.19	&	0.08 $\pm$ 0.24	&	3	\\
13	&	IRAS14429-4539	&	–0.18 $\pm$ 0.11	&	1.29 $\pm$ 0.26	&	0.31 $\pm$ 0.12	&	0.68 $\pm$ 0.23	&	\nodata	&	1.41 $\pm$ 0.08	&	\nodata	&	1.46 $\pm$ 0.17	&	1.29 $\pm$ 0.15	&	1.47 $\pm$ 0.10	&	0.18 $\pm$ 0.08	&	3	\\
14	&	IRAS19500-1709	&	–0.59 $\pm$ 0.10	&	1.02 $\pm$ 0.17	&	0.72 $\pm$ 0.04	&	0.99 $\pm$ 0.06	&	0.41 $\pm$ 0.30	&	1.35 $\pm$ 0.21	&	\nodata	&	1.34 $\pm$ 0.10	&	1.37 $\pm$ 0.29	&	1.34 $\pm$ 0.30	&	–0.03 $\pm$ 0.41	&	3	\\
15	&	IRAS20000+3239	&	-1.4 $\pm$ 0.2	&	\nodata	&	\nodata	&	1.7 $\pm$ 0.2	&	2.1 $\pm$ 0.2	&	1.4 $\pm$ 0.2	&	\nodata	&	1 $\pm$ 0.2	&	1.1 $\pm$ 0.2	&	1.47 $\pm$ 0.10	&	0.34 $\pm$ 0.2	&	5	\\
16	&	IRAS22223+4327	&	–0.30 $\pm$ 0.11	&	1.04 $\pm$ 0.22	&	0.31 $\pm$ 0.06	&	0.59 $\pm$ 0.06	&	0.15 $\pm$ 0.30	&	1.03 $\pm$ 0.05	&	0.12 $\pm$ 0.08	&	1.35 $\pm$ 0.06	&	1.34 $\pm$ 0.07	&	0.88 $\pm$ 0.07	&	–0.46 $\pm$ 0.10	&	3	\\
17	&	IRAS22272+5435	&	–0.77 $\pm$ 0.12	&	1.46 $\pm$ 0.26	&	0.63 $\pm$ 0.02	&	1.05 $\pm$ 0.07	&	\nodata	&	1.80 $\pm$ 0.05	&	0.28 $\pm$ 0.02	&	1.54 $\pm$ 0.08	&	1.61 $\pm$ 0.08	&	1.90 $\pm$ 0.07	&	0.28 $\pm$ 0.11	&	3	\\
18	&	IRAS23304+6147	&	−0.81 $\pm$ 0.2	&	2.8 $\pm$ 0.2	&	0.17 $\pm$ 0.03	&	0.91 $\pm$ 0.12	&	0.47 $\pm$ 0.15	&	1.60 $\pm$ 0.25	&	0.44 $\pm$ 0.13	&	1.26 $\pm$ 0.23	&	1.55 $\pm$ 0.23	&	1.63 $\pm$ 0.21	&	0.09 $\pm$ 0.24	&	6	\\
\hline
\multicolumn{14}{c}{Post-AGB stars without $s$-process enrichment}\\
\hline
19	&	IRAS01259+6823	&	-0.60 $\pm$ 0.1	&	0.4 $\pm$ 0.3	&	0.31 $\pm$ 0.06	&	0.18 $\pm$ 0.3	&	\nodata	&	0.3 $\pm$ 0.1	&	\nodata	&	0.12 $\pm$ 0.1	&	\nodata	&	\nodata	&	\nodata	&	7	\\
20	&	IRAS08187-1905	&	-0.60 $\pm$ 0.1	&	\nodata	&	0.26 $\pm$ 0.1	&	0.62 $\pm$ 0.3	&	0.49 $\pm$ 0.3	&	\nodata	&	0.64 $\pm$ 0.1	&	0.25 $\pm$ 0.1	&	\nodata	&	\nodata	&	\nodata	&	7	\\
21	&	SAO239853	&	-0.81 $\pm$ 0.1	&	\nodata	&	0.8 $\pm$ 0.2	&	0.4 $\pm$ 0.2	&	0.6 $\pm$ 0.2	&	-0.4 $\pm$ 0.2	&	0.4 $\pm$ 0.2	&	\nodata	&	\nodata	&	\nodata	&	\nodata	&	8	\\
22	&	HD107369	&	-1.1 $\pm$ 0.1	&	\nodata	&	0 $\pm$ 0.2	&	<-0.2	&	0.49 $\pm$ 0.3	&	-0.1 $\pm$ 0.2	&	0.1 $\pm$ 0.2	&	\nodata	&	\nodata	&	\nodata	&	\nodata	&	8	\\
23	&	HD112374	&	-1.2 $\pm$ 0.1	&	\nodata	&	0.8 $\pm$ 0.2	&	0.1 $\pm$ 0.2	&	0.5 $\pm$ 0.2	&	-0.3 $\pm$ 0.2	&	0.1 $\pm$ 0.2	&	\nodata	&	\nodata	&	\nodata	&	\nodata	&	8	\\
24	&	HD133656	&	-0.7 $\pm$ 0.1	&	\nodata	&	0.6 $\pm$ 0.2	&	0.3 $\pm$ 0.2	&	0.5 $\pm$ 0.2	&	-0.4 $\pm$ 0.2	&	0.4 $\pm$ 0.2	&	\nodata	&	\nodata	&	\nodata	&	\nodata	&	8	\\
25	&	HR6144	&	-0.4  $\pm$ 0.1	&	\nodata	&	0.3 $\pm$ 0.2	&	0.3 $\pm$ 0.2	&	0.9 $\pm$ 0.2	&	0.2 $\pm$ 0.2	&	0.4 $\pm$ 0.2	&	\nodata	&	\nodata	&	\nodata	&	\nodata	&	8	\\
26	&	HD161796	&	-0.3 $\pm$ 0.1	&	\nodata	&	0.4 $\pm$ 0.2	&	0.3 $\pm$ 0.2	&	1.1 $\pm$ 0.2	&	0 $\pm$ 0.2	&	0.7 $\pm$ 0.2	&	\nodata	&	\nodata	&	\nodata	&	\nodata	&	8	\\
27	&	IRAS18025-3906	&	-0.51 $\pm$ 0.15	&	0.43	&	0.56 $\pm$ 0.2	&	0.46 $\pm$ 0.2	&	0.74 $\pm$ 0.2	&	\nodata	&	0.88 $\pm$ 0.1	&	-0.84 $\pm$ 0.04	&	\nodata	&	\nodata	&	\nodata	&	9	\\
28	&	HD335675	&	-0.9 $\pm$ 0.2	&	0.25	&	0.77 - 0.19	&	0.4 - 0.35	&	$<$0.27 	&	\nodata	& 0.77 $\pm$ 0.02	&	-0.36 $\pm$ 0.1	&	\nodata	&	\nodata	&	\nodata	&	10	\\
29	&	IRAS19386+0155	&	-1.1 $\pm$ 0.14	&	\nodata	&	\nodata	&	0.1 $\pm$ 0.2	&	\nodata	&	-0.3 $\pm$ 0.2	&	\nodata	&	\nodata	&	\nodata	&	\nodata	&	\nodata	&	11	\\
30	&	IRAS19475+3119	&	−0.24 $\pm$ 0.15	&	0.19	&	0.30 $\pm$ 0.02	&	-0.09 $\pm$ 0.30	&	\nodata	&	-0.30 $\pm$ 0.1	&	0.53 $\pm$ 0.18	&	\nodata	&	\nodata	&	\nodata	&	\nodata	&	12	\\
31	&	HR7671	&	-1.6 $\pm$ 0.1	&	0.05	&	0.46 $\pm$ 0.05	&	-0.57 $\pm$ 0.13	&	0.51 $\pm$ 0.16	&	\nodata	&	0.29 $\pm$ 0.06	&	0.44 $\pm$ 0.15	&	\nodata	&	\nodata	&	\nodata	&	13	\\
\enddata
\tablenotetext{*}{\textbf{Note: The index \sfe\, is the mean of the relative abundances of the elements for the 'ls' and 'hs' indices. Typically, the 'ls' index uses the mean of the relative abundances of Y and Zr and the 'hs' index uses the mean of the relative abundances of La, Ce, Nd and Sm. \hsls\,. More details on the derived abundances and abundance ratios can be found in the individual studies mentioned in column 'Ref'}. The column 'Ref.' indicates the individual chemical abundance study: $^{1}$\cite{reddy99}, $^{2}$\cite{vanwinckel00}, $^{3}$\cite{desmedt16}, $^{4}$\cite{pereira11}, $^{5}$\cite{klochkova06}, $^{6}$\cite{ReyniersThesis}, $^{7}$\cite{rao12}, $^{8}$\cite{vanwinckel97a}, $^{9}$\cite{molina19}, $^{10}$\cite{sahin11}, $^{11}$\cite{pereira04}, $^{12}$\cite{arellanoferro01}, $^{13}$\cite{reyniers05}.}
%\tablecomments{}
\end{deluxetable*}
\end{longrotatetable}

